DICE: Automatic Emulation of DMA Input Channels for Dynamic Firmware Analysis

Microcontroller-based embedded devices are at the core of Internet-of-Things and Cyber-Physical Systems. The security of these devices is of paramount importance. Among the approaches to securing embedded devices, dynamic firmware analysis gained great attention lately, thanks to its offline nature and low false-positive rates. However, regardless of the analysis and emulation techniques used, existing dynamic firmware analyzers share a major limitation, namely the inability to handle firmware using DMA. It severely limits the types of devices supported and firmware code coverage. We present DICE, a drop-in solution for firmware analyzers to emulate DMA input channels and generate or manipulate DMA inputs. DICE is designed to be hardware-independent, and compatible with common MCU firmware and embedded architectures. DICE identifies DMA input channels as the firmware writes the source and destination DMA transfer pointers into the DMA controller. Then DICE manipulates the input transferred through DMA on behalf of the firmware analyzer. We integrated DICE to the firmware analyzer P2IM (Cortex-M architecture) and a PIC32 emulator (MIPS M4K/M-Class architecture). We evaluated it on 83 benchmarks and sample firmware, representing 9 different DMA controllers from 5 different vendors. DICE detected 33 out of 37 DMA input channels, with 0 false positives. It correctly supplied DMA inputs to 21 out of 22 DMA buffers, which previous firmware analyzers cannot achieve due to the lack of DMA emulation. DICE's overhead is fairly low, it adds 3.4% on average to P2IM execution time. We also fuzz-tested 7 real-world firmware using DICE and compared the results with the original P2IM. DICE uncovered tremendously more execution paths (as much as 79X) and found 5 unique previously-unknown bugs that are unreachable without DMA emulation. All our source code and dataset are publicly available.

==> Makefile <==
# Set this to one or more main LaTeX files (e.g. those with \documentclass) 
# for a specific build. Leave blank to build all files having an uncommented
# \documentclass.
MAIN=main.tex	


###########################################################################
#                 MAKE NO EDITS BELOW (except to debug)                   #
###########################################################################
#
#
# This is the PDFLATEX makefile, no support for ps/eps/dvi.
#
# Originally based on 
#   http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/Makefile
# but redeveloped by JG. Reuse by changing just the first line to list
# the main LaTeX source file.
#
# Features:
# - Finds all included LaTeX files, including includes within includes.
# - Finds all bibs and PDF figures included.
# - Automatically generates dependency information.
# - Repeats calls to PDFLATEX as necessary to fix cross references.
# - Displays missing references in a clean format at the end of the build.
# - Finds main LaTeX source files, so this makefile is reusable wihtout edits.
# - Works for files with bibliographies, and files without.

ifndef MAIN
MAIN:=	$(shell egrep -l "documentclass" *.tex)	
endif

ALLTEX:=$(shell ls *.tex)
ALLPDF:=$(ALLTEX:.tex=.pdf)

all pdf: $(MAIN:.tex=.pdf)
help ps dvi $(MAIN:.tex=.ps) $(MAIN:.tex=.dvi): die_unsupported
$(filter-out $(MAIN:.tex=.pdf),$(ALLPDF)): die_unsupported

%.pdf: %.fig
	rm -f $@
	fig2dev -L pdf $< > $@

%.aux: %.tex
	$(LATEX) $<

%.bbl: %.tex
	bibtex $(<:.tex=)
	$(LATEX) $<

%.pdf: %.aux
	@while (grep -q "Rerun to get" $(<:.aux=.log)) do \
		$(LATEX) $(<:.aux=.tex); \
	done
	@egrep -i "(Reference|Citation).*undefined" $(<:.aux=.log) ; true
	$(LATEX) $(<:.aux=.tex)

%.dep: %.tex
	@$(gettexs); $(getbibs); $(getfigs); \
	echo "$(<:.tex=.dep): Makefile " $$texs $$bibs $$figs > $@; \
	echo "$(<:.tex=.aux): " $$texs $$figs >> $@; \
	if [ $${#bibs} -gt 0 ]; then \
		echo "$(<:.tex=.bbl): " $$texs $$bibs >> $@; \
		echo "$(<:.tex=.pdf): $(<:.tex=.bbl)" >> $@; \
	fi

vpath %.fig figs

-include $(MAIN:.tex=.dep)

.PHONY: clean die_unsupported

double:
	for i in $(ALLTEX); do echo "Double words in $$i:" && ./double.pl < $$i; done

clean:
	rm -f *~ *.log *.aux *.dvi *.bbl *.blg *.cb *.dep $(TARGET)

die_unsupported:
	$(warning Unsupported Makefile build target. Supported targets are:)
	$(warning  <BLANK> all pdf $(TARGET) clean)
	$(error Exiting)

LATEX=	pdflatex #--interaction batchmode
TARGET=	$(MAIN:.tex=.pdf)

# 9 Dec 2008 JG: This is now a worklist algorithm to pick up all recursive
#   child dependencies of discovered includes.
define gettexs
  worklist="$< "; \
  while [ $${#worklist} -gt 0 ]; do \
    curr=$${worklist%% *}; \
    worklist=$${worklist#* }; \
    texs="$${texs}$$curr "; \
    worklist=$${worklist}`perl -ne '\
               ($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/; \
	       @_=split /,/; \
	       foreach $$t (@_) { \
	         if ($$t !~ /\.tex$$/) { $$t .= ".tex"; } \
                 if (-e $$t) { print "$$t " } \
	       }' $${curr}`; \
	done
endef

define getbibs
  bibs=`perl -ne '\
        ($$_)=/^[^%]*\\\bibliography\{(.*?)\}/; \
        @_=split /,/; \
        foreach $$b (@_) { \
          if (-e "$$b.bib") { print "$$b.bib " } \
        }' $$texs`
endef

define getfigs
  figs=`perl -ne '\
        ($$_)=/^[^%]*\\\includegraphics(?:\[.*?\])?\{(.*?)\}/g; \
        if (defined($$_)) { \
          if ($$_ !~ /\.pdf$$/) { $$_ .= ".pdf"; } \
          if (-e $$_) { print "$$_ "; } \
        }' $$texs`
endef


==> overview.tex <==
\section{Overview}
